Searching for Decoherence from Quantum Gravity at the IceCube South Pole Neutrino Observatory

Neutrino oscillations at the highest energies and longest baselines provide a natural quantum interferometer with which to study the structure of spacetime and test the fundamental principles of quantum mechanics. If the metric of spacetime has a quantum mechanical description, there is a generic expectation that its fluctuations at the Planck scale would introduce non-unitary effects that are inconsistent with the standard unitary time evolution of quantum mechanics. Neutrinos interacting with such fluctuations would lose their quantum coherence, deviating from the expected oscillatory flavor composition at long distances and high energies. The IceCube South Pole Neutrino Observatory is a billion-ton neutrino telescope situated in the deep ice of the Antarctic glacier. Atmospheric neutrinos detected by IceCube in the energy range 0.5--10 TeV have been used to test for coherence loss in neutrino propagation. No evidence of anomalous neutrino decoherence was observed, leading to the strongest experimental limits on neutrino-quantum gravity interactions to date, significantly surpassing expectations from natural Planck-scale models. The resulting constraint on the effective decoherence strength parameter within an energy-independent decoherence model is $\Gamma_0\leq 1.17\times10^{-15}$~eV, improving upon past limits by a factor of 30. For decoherence effects scaling as E$^2$, limits are advanced by more than six orders of magnitude beyond past measurements.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


